TIDE: A General Toolbox for Identifying Object Detection Errors

We introduce TIDE, a framework and associated toolbox for analyzing the sources of error in object detection and instance segmentation algorithms. Importantly, our framework is applicable across datasets and can be applied directly to output prediction files without required knowledge of the underlying prediction system. Thus, our framework can be used as a drop-in replacement for the standard mAP computation while providing a comprehensive analysis of each model's strengths and weaknesses. We segment errors into six types and, crucially, are the first to introduce a technique for measuring the contribution of each error in a way that isolates its effect on overall performance. We show that such a representation is critical for drawing accurate, comprehensive conclusions through in-depth analysis across 4 datasets and 7 recognition models. Available at https://dbolya.github.io/tide/

==> figures/1_error_examples.tex <==
\begin{figure}[t]
    \begin{center}

    \newcommand{\errorexample}{\subfloat{{\includegraphics[width=1.75cm,height=5.5cm]{example-image-a} }} \,\,}
    
    \begin{tabular}{c: c: c: c: c: c}
         \small{\textbf{Cls}} & \small{\textbf{Loc}} &
        \small{\textbf{Cls+Loc}} & 
        \small{\textbf{Duplicate}} & 
        \small{\textbf{Bkgd}} & 
        \small{\textbf{Missed}}\\
        \midrule
        \includegraphics[width=.16\linewidth]{figures/error_types/err_classification.png} &  
        \includegraphics[width=.16\linewidth]{figures/error_types/err_localization.png} &
        \includegraphics[width=.16\linewidth]{figures/error_types/err_both.png} &
        \includegraphics[width=.16\linewidth]{figures/error_types/err_duplicate.png} &
        \includegraphics[width=.16\linewidth]{figures/error_types/err_bkgnd.png} &
        \includegraphics[width=.16\linewidth]{figures/error_types/err_missed.png} \\
        \includegraphics[width=.16\linewidth]{figures/error_types/Iou_classification.pdf}%\small{$t_f \leq IoU$}
        &\small{ $t_{b} < IoU < t_{f}$}
        & \small{$t_{b} < IoU < t_{f}$}
        & \small{$t_{f} < IoU $}
        & \small{$IoU < t_{b} $}
        & \small{NA}
    \end{tabular}
    
    %\errorexample
    %\errorexample
    %\errorexample
    %\errorexample
    %\errorexample
    %\errorexample
    
    \end{center}
    \caption{\textbf{Error Type Definitions.} Qualitative examples for each of the 6 error types in Mask R-CNN on COCO. For each error type, we choose the three highest scoring detections that aren't a result of poor annotation. }
    
    \label{fig:1_error_examples}
\end{figure}
